Probing Factually Grounded Content Transfer with Factual Ablation

Despite recent success, large neural models often generate factually incorrect text. Compounding this is the lack of a standard automatic evaluation for factuality--it cannot be meaningfully improved if it cannot be measured. Grounded generation promises a path to solving both of these problems: models draw on a reliable external document (grounding) for factual information, simplifying the challenge of factuality. Measuring factuality is also simplified--to factual consistency, testing whether the generation agrees with the grounding, rather than all facts. Yet, without a standard automatic metric for factual consistency, factually grounded generation remains an open problem. We study this problem for content transfer, in which generations extend a prompt, using information from factual grounding. Particularly, this domain allows us to introduce the notion of factual ablation for automatically measuring factual consistency: this captures the intuition that the model should be less likely to produce an output given a less relevant grounding document. In practice, we measure this by presenting a model with two grounding documents, and the model should prefer to use the more factually relevant one. We contribute two evaluation sets to measure this. Applying our new evaluation, we propose multiple novel methods improving over strong baselines.

==> figs/fig_cf_synth.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|ccc|}
     \toprule
       & acc & acc-margin & margin \\ 
   \midrule
      \rowcolor[gray]{0.95}
   \multicolumn{4}{l}{\emph{Zero Shot and Transfer}}  \\
   factcc (mean) & 70.1 & - & - \\
   factcc (max) & 37.0 & - & - \\
   gpt2-zs & 78.0 & 2.4 & 0.9\\
   \midrule
   \rowcolor[gray]{0.95}
   \multicolumn{4}{l}{\emph{Tuned}} \\
   hotstart & 74.4 & 10.7 & 1.7 \\
   tuned & 75.0 & 19.6 & 2.5\\
    \midrule
    \rowcolor[gray]{0.95}
    \multicolumn{4}{l}{\emph{Loss Truncation}} \\
   $LT_{basic}$ & 75.0 & 23.8 & 2.5 \\
   $LT_{+gnd}$ & 75.0 & 18.5 & 2.3 \\
   \midrule
   \rowcolor[gray]{0.95}
   \multicolumn{4}{l}{\emph{Inference-time}}\\
   $P_{pmi interp}$ alpha 0.1 & 75.0 & 20.8 & 2.5 \\
   $P_{pmi interp}$ alpha 0.3 & 75.0 & 21.4 & 2.5 \\
   $P_{pmi interp}$ alpha 0.5 & 76.8 & 23.8 & 2.8 \\
   \midrule
   $P_{pmi add}$ alpha 0.1 & 74.4 & 23.8 & 2.6 \\
   $P_{pmi add}$ alpha 0.3 & 73.2 & 28.6 & 2.9 \\
   $P_{pmi add}$ alpha 0.5 & 71.4 & 32.1 & 3.2 \\
     \bottomrule
    \end{tabular}
    \caption{Evaluation of model preference for correct grounding when generating target. This is on our \emph{synthetic} dataset based on manual edits to grounding and target. \emph{acc} is raw accuracy, \emph{acc-margin} requires correct prediction by a given margin (likelihood at least 100 time higher) and \emph{margin} is average difference in NLL between correct and incorrect grounding.
    }  
    \label{tab:cg_synth}
\end{table}

==> figs/fig_cf_wiki.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|ccc|}
     \toprule
       & acc & acc-margin & margin \\ 
   \midrule
   \rowcolor[gray]{0.95}
   \multicolumn{4}{l}{\emph{Zero Shot and Transfer}}  \\
   factcc (mean) & 30 & - & - \\
   factcc (max) & 63.9 & - & - \\
   gpt2-zs & 84.5 & 54.5 & 12.4 \\
   \midrule
      \rowcolor[gray]{0.95}
   \multicolumn{4}{l}{\emph{Tuned}} \\
   hotstart & 87.9 & 64.5 & 16.9 \\
   tuned & 87.7 & 69.2 & 19.4\\
    \midrule
    \rowcolor[gray]{0.95}
    \multicolumn{4}{l}{\emph{Loss Truncation}} \\
   $LT_{basic}$ & 87.7 & 70.3 & 20.2 \\
   $LT_{+gnd}$ & 88.2 & 71.1 & 21.0 \\
   \midrule
   \rowcolor[gray]{0.95}
   \multicolumn{4}{l}{\emph{Inference-time}}\\
   $P_{pmi interp}$ alpha 0.1 & 88.0 & 69.0 & 19.6\\
   $P_{pmi interp}$ alpha 0.3 & 88.6 & 71.3 & 21.5\\
   $P_{pmi interp}$ alpha 0.5 & 88.9 & 76.1 & 26.2\\
   \midrule
   $P_{pmi add}$ alpha 0.1 & 87.9 & 70.6 & 20.2\\
   $P_{pmi add}$ alpha 0.3 & 87.9 & 72.7 & 21.8\\
   $P_{pmi add}$ alpha 0.5 & 87.3 & 73.0 & 23.2 \\
     \bottomrule
    \end{tabular}
    \caption{Evaluation of model preference for correct grounding when generating target. This is on our \emph{natural} dataset based on Wikipedia edits. \emph{acc} is raw accuracy, \emph{acc-margin} requires correct prediction by a given margin (likelihood at least 1000 time higher) and \emph{margin} is average difference in NLL between correct and incorrect grounding.
    }  
    \label{tab:cf_wiki}
\end{table}

==> figs/fig_data_stats.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|cc}
     \toprule
     & CT & Counterfactual\\
     \midrule

   total examples & X & X  \\
   News Domains & Y & Y  \\
   Target Length & - & - \\
   Context Length & - & - \\
   Document Length & - & - \\

     \bottomrule
    \end{tabular}
    \caption{Comparison of our counterfactual evaluation set with the content transfer dataset. NOTE: give basic picture of our set, and demonstrate its relationship with CT}  
    \label{tab:data_stats}
\end{table}

==> figs/table_example_0.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{p{0.9\linewidth}} %{l|l|}
     \toprule
     \rowcolor[gray]{0.95}
     Grounding \\
   SOUTH PASADENA, Calif., March 31 (AP)--Ralph De Palma, pioneer auto racer who probably won more races than any other driver in history, died today of cancer. His age was 72. ...\\
   \midrule
   \rowcolor[gray]{0.95}
   Context\\
   Speedway management would maintain their policy to not race on Sundays until 1974 Indianapolis 500|1974. After a heartbreaking loss in 1912 Indianapolis 500|1912, Ralph DePalma succeeds in victory for 1915. DePalma was accompanied by riding mechanic Louis Fontaine.\\
   \midrule
   \midrule
   \rowcolor[gray]{0.95}
   Next sentence  \\
   \midrule
   \textit{GPT-3}: The \textbf{1915} race was the first to have a post-race distance of more than \underline{500 miles}. \\
   \midrule
   \textit{GPT-2}$_{tuned}$: depalma \textbf{died on march 31}, \underline{1915}, \textbf{at his home in south pasadena, california}, of \textbf{cancer}. \\
   \midrule
   \textit{GPT-2}$_{LT}$: \underline{he was the first driver to win} the world war i era american championship. \\
   \midrule
   \textit{GPT-2}$_{pmi-add}$: \textbf{depalma died of cancer at his home in south pasadena, california, at the age of 72.} \\
     \bottomrule
    \end{tabular}
    \caption{Generation with different models continuing a wikipedia article. GPT-3 has no grounding, while the other 3 models
    use one document as grounding. The table highlights  \textbf{factual} and \underline{false} information. }
    %We bold \textbf{factual information} and underline \underline{false information}.}
     
    \label{tab:example_0}
\end{table}

==> sections/data.tex <==
\section{Data}
\label{sec:data}

%\peter{mention why it's important to do small ablations (i.e. not just pick a random adversarial document. Because if we can do it automatically, it's probably way too easy, and if it's too close it's not clear that it will meet the factual ablation condition, might be inverted).}


\subsection{Content Transfer}
\label{subsec:data_content_transfer}

The task of \promptTask was introduced by \citet{prabhumoye2019towards}, with a dataset using Wikipedia articles to extract context and target, and external references as grounding. An example $(g,c,y)$ consists of a sentence $y$ from Wikipedia (including a reference), the preceding sentences $c$ serving as a prompt, and the external document $g$ referenced by $y$, containing its factual basis. Quality of grounding documents $g$ was ensured by filtering to only include web pages from a set of trusted news sites, and further processing for quality.

\citet{prabhumoye2019towards} release a dataset with 600K training examples, 6K validation examples, and 50K test examples. We train using this data, and use their evaluation set as the basis for our generations used for lexical and human evaluation. Measuring factual ablation on this original dataset is not an option as there is only one piece of grounding per-example, and so we describe two paths to generating evaluation data for this purpose below.

\subsection{Synthetic Factual Ablation}
\label{subsec:data_synthetic}

Deliberate and purposeful edits offer a simple path to evaluating aspects of models \citep{Ribeiro2020BeyondAB}. As such, one approach we offer for generating evaluation data for factual ablation is using handcrafted examples. By making point-edits to the grounding document $g$ to produce $g'$ which has strictly fewer facts in common with target $y$, we can easily produce correct and interpretable factual ablation examples. 

We construct a set of synthetic examples by editing single pieces of information in both the grounding $g$ and target $y$, producing $g'$ and $y'$ which share this modified fact. This yields two examples:

$$(g,g',c,y)\text{ and } (g',g,c,y')$$
\noindent
where $y$ should prefer $g$ and $y'$ should prefer $g'$. We limit edits to two types of information: numerical (changing numbers: e.g., four miners became stuck $\xrightarrow{}$ two miners became stuck) and chronological (the Queen toured Canada in March $\xrightarrow{}$ the Queen toured Canada in April). These edits are only made for examples where (i) the fact is not commonly known, (ii) changing it does not violate any obvious commonsense restrictions and (iii) the fact appears in both the grounding $g$ and target $y$. Our resulting dataset contains 162 such examples (see appendix for example). Note, from an ethical standpoint we avoid constructing examples related to sensitive topics or potential disinformation. Synthetic factual ablation is useful at a small scale, but should not be done at a large scale for this reason.

While synthetic data is simple to produce and well-controlled, it has obvious drawbacks. Mainly, the style of factual differences produced will be limited and biased, and the number of example will be relatively low as each must be handcrafted. To overcome these issues, we also introduce a natural evaluation set.


\subsection{Natural Factual Ablation}
\label{subsec:data_wiki}
The use of Wikipedia data for the original \promptTask dataset from \citet{prabhumoye2019towards} offers an intuitive way to construct natural evaluation  data for factual ablation. Because Wikipedia is constantly being edited, there are many instances where one sentence $y$ including a reference $g$, is replaced by another pair $y'$, $g'$. In practice, $y,y'$ will tend to be \textit{entailed} by their own grounding ($g,g'$ respectively) and not the reverse. This means $g$ can serve as ablated grounding for $y'$ and vice versa. We are also ensured that both $g,g'$ can result in a reasonable continuation to $c$, which ensures that examples are not trivial. Selecting such a document automatically would be challenging: if it is too unrelated the example it becomes trivial, while a relevant document may not be considered ablated at all (i.e., it may contain as much relevant information as the original). 
%
The Wikipedia-edit dataset is constructed as follows:

\begin{enumerate}[nosep]
    \item Isolate all instances $(g,g',c,y,y')$ in Wikipedia edit data where referenced sentence $y$ has been replaced by referenced sentence $y'$.
    \item From each such instance, construct two \measure examples: $(g,g',c,y)$ and $(g',g,c,y')$.
    \item Filter any such examples that do not meet quality criteria.
\end{enumerate}

We impose a number of quality criteria on examples $(g,g', c,y)$. These include: $y$ is within a reasonable length range, $g$ and $g'$ come from news sites and can be fully recovered, no text includes excessive formatting issues. We will release processing code with the dataset. We attempt to recreate a similar distribution to the \promptTask dataset of \citet{prabhumoye2019towards}, following the same post processing steps. This is important to prevent major domain transfer issues between our training and testing. In total, we extract 710 examples, although larger sets can be constructed as Wikipedia is constantly being edited. See appendix for a full example. 
